Online Prediction with Selfish Experts

We consider the problem of binary prediction with expert advice in settings where experts have agency and seek to maximize their credibility. This paper makes three main contributions. First, it defines a model to reason formally about settings with selfish experts, and demonstrates that "incentive compatible" (IC) algorithms are closely related to the design of proper scoring rules. Designing a good IC algorithm is easy if the designer's loss function is quadratic, but for other loss functions, novel techniques are required. Second, we design IC algorithms with good performance guarantees for the absolute loss function. Third, we give a formal separation between the power of online prediction with selfish experts and online prediction with honest experts by proving lower bounds for both IC and non-IC algorithms. In particular, with selfish experts and the absolute loss function, there is no (randomized) algorithm for online prediction-IC or otherwise-with asymptotically vanishing regret.

==> conclusion.tex <==
\section{Conclusion}
\label{s:conclusion}
In this paper we showed three things.
The first contribution of this paper is the development of a model for
reasoning formally about the design and analysis
of weight-based online prediction
algorithms when experts are selfish, and the
definition of an ``incentive-compatible'' (IC) such algorithm.
We demonstrated that the design of IC online
prediction algorithms is closely related to the design of strictly
proper scoring rules. Using this, we showed that for the quadratic loss
function, the standard WM and RWM
algorithms give good guarantees, whereas these algorithms are not
generally incentive compatible for other loss functions.

Our second contribution is the design of IC
prediction algorithms for the absolute loss function with non-trivial performance guarantees.  For
example, our best result for deterministic algorithms is: the WM
algorithm, with experts' weights evolving according to the spherical
proper scoring rule, is IC
and has loss at most $2+\sqrt{2}$ times the loss of best
expert in hindsight (in the limit as $T \rightarrow \infty$).  A
variant of the RWM algorithm with the Brier scoring rule is IC and has expected loss at most 2.62 times that of
the best expert in hindsight (also in the limit).

Our third and most technical contribution is
formal separation between online prediction with selfish experts and the traditional setting with honest experts.
Recall that with honest experts, the classical (deterministic) WM
algorithm has loss at most twice that of the best expert in hindsight
(as $T \rightarrow \infty$).  We prove that the worst-case loss of
every (deterministic) IC algorithm  also every
non-IC algorithm satisfying mild technical conditions has worst-case loss bounded away from
twice that of the best expert in hindsight (even as
$T \rightarrow \infty$).  A consequence of our lower bound is that,
with selfish experts, there is no natural (randomized) algorithm for
online prediction---IC or otherwise---with asymptotically vanishing
regret.

%\paragraph{Open Problems}

% tight bounds (we still have a fairly large gap now)

% characterization of the cost of selfish experts based on parameters of the strictly proper scoring rule

% going beyond the binary outcome case

%Ideas: In \cite{BD89} the authors discuss different objective functions for experts, including trying to optimize relative weight among different experts under different informational assumptions. These would impose different constraints as to which algorithms would lead to truthful reporting, and it would be interesting to see if no-regret learning is possible in this setting.

% Bandit setting

==> related.tex <==
\paragraph{Related Work}
We believe that our model of online prediction over time with selfish
experts is novel.  We next survey the multiple other ways in which online
learning and incentive issues have been blended in previous works.

There is a large literature on prediction and decision markets
(e.g.~\cite{chen_pennock10,horn14}), which also aim to aggregate
information over time from multiple parties and make use of proper
scoring rules to do it.  There are several major differences between
our model and prediction markets.  First, in our model, the goal is to
predict a sequence of events, and there is feedback (i.e., the
realization) after each one.  In a prediction market, the goal is to
aggregate information about a single event, with feedback provided
only at the end (subject to secondary objectives, like bounded
loss).\footnote{In the even more distantly related peer prediction
scenario~\citep{MRZ05}, there is never any realization at all.}
Second, our goal is to make accurate predictions, while that of a
prediction market is to aggregate information.  For example, if
one expert is consistently incorrect over time, we would like to
ignore her reports rather than aggregate them with others' reports.
Third, in the dominant paradigm in prediction market design,
participants express their beliefs by
buying and selling securities managed by a market-maker, and act to
maximize their expected profit.  In our model, participants directly
declare their beliefs to a weight-update-based prediction algorithm,
no money changes hands, and experts are motivated by their weight
assigned by the algorithm.
Finally, while there are strong mathematical connections between cost
function-based prediction markets and regularization-based online
learning algorithms in the standard (non-IC) model~\citep{ACV12}, there
does not appear to be any interesting implications for online
prediction with selfish experts.

There is also an emerging literature on ``incentivizing exploration''
(as opposed to exploitation) in partial feedback models such as the
bandit model (e.g.~\cite{FKKK14,MSSW16}).  Here, the incentive issues
concern the learning algorithm itself, rather than the experts (or
``arms'') that it makes use of.

%\os{Tim, see the folder ``Spring14'' for more related work and citations.}

% {\bf Proper scoring rules}
% \os{Should we define (strictly) proper scoring rules here?}
% \cite{B50} started the field of proper scoring rules. \cite{S71} gave (the first?) general characterization for proper scoring rules. \cite{GR07} is a recent survey of the field.
% \cite{B05} look at using proper scoring rules as loss functions in learning. differences with us: we assume selfish reports and a multiplicative objective function, not additive.
% Less relevant is \cite{MS13} who look at choosing a strictly proper scoring rule to fit a particular goal (this is what I've been looking at trying to reduce the apx factors).

% %xxx yishay says: 
% A long time ago I worked with Nicolo Cesa-Bianchi and Fabrizio Germano
% on experts  
% that have a different loss for false positive and false negative.
% This has a literature in economics under decision making (jury
% selection as a motivation).
% For the one-shoot scenario they have impossibility results.
% I vaguely recall Andrew Postlewaite as one of the co-authors (hope my
% memory is correct).
% Probably it is the following:
% ``Aggregation of Expert Opinions” (D. Gerardi, R. McLean,
% Postlewaite, A.), Games and Economic Behavior, 2008, 65(2): 339-371.
% There are many more works in economics on aggregation of expert
% opinions.
% There is also strategic manipulation of tests (Sandroni and others,
% basically showing that you can fool any test)

% we tried to get around the impossibility in a repeated setting.
% We basically has ``folk theorems'' where the principal can punish the
% experts for making mistakes.
% We had some abstract in GAMES 2011 (could not recover the draft
% easily, but we did not have much ...)
% Our focus, like much of the economics literature was on the
% aggregation part.
% Unfortunately there is too much related work (hard to know where to
% start)

% On a similar topic, at some point I tried to show that a single
% malicious expert cannot do too much harm if you do exponential
% weights, since it has to balance its weight (derived by its accuracy)
% and the errors it inflicts.
% Unfortunately such an expect cannot do too much harm, since we are
% guarantee by the regret minimization to match the bets expert,
% which is either him (great!) or someone else. He can probably increase
% the regret from zero to sqrt{T}. Not sure if it is interesting.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "selfish-experts"
%%% End:


==> scoring.tex <==
\section{Proper Scoring Rules and IC Learning}
\label{s:scoring}

Lemma~\ref{lem:myopic} shows the myopically responding at each time $t$ is the optimal strategy for each expert, but this doesn't yet tell us what that report will be. In fact, in Example~\ref{ex:obvious} we already saw that the best response may not be the true belief $\bt$ of the expert. In this section we show a tight correspondence between truthful reporting at each time step and (strictly) proper scoring rules. Since we are interested in predicting binary events, we look at binary proper scoring rules.

\begin{definition}[Binary Proper Scoring Rule, \cite{GR07}]
	\label{def:psr}
	A function $f : [0,1]\times\{0,1\}\rightarrow \R\cup \{\pm\infty\}$ is a binary proper scoring rule if it is finite except possibly on its boundaries and whenever for $p, q \in [0,1]$
	$$p \in \max_q p\cdot f(q, 1) + (1-p)\cdot f(q, 0).$$
\end{definition}

Intuitively, one could consider $p$ as the true probability of event $1$ materializing, and $q$ the report. Function $f$ is a proper scoring rule when reporting the true probability maximizes the expected score. Moreover a function $f$ is a \emph{strictly} proper scoring rule if $p$ is the only value that maximizes the expectation.

We call a weight update function $f$ incentive compatible (IC) if reporting the true belief $\bt$ is a best response for each expert. Furthermore it is strictly IC when $\pt = \bt$ is the only best-response.

\begin{theorem}
	\label{thm:psr}
	A weight update rule is (strictly) incentive compatible if and only if $f$ is a (strictly) proper scoring rule.
\end{theorem}
\begin{proof}
	By Lemma~\ref{lem:myopic} we know that the expert will maximize the expected value for her report $\pt$ with respect to her beliefs: $\pt \in \max_p \E_r f(p, r)$. The set of functions $f$ for which $\bt\in\max_p \E_r f(p, r)$ is the set of proper scoring rules. So $\bt$ is a weakly dominant strategy when $f$ is a proper scoring rule. The set of functions for which $\bt=\max_p \E_r f(p, r)$ is the set of strictly proper scoring rules. So the weight update rule is (strictly) incentive compatible if and only $f$ is a (strictly) proper scoring rule.
\end{proof}


So when considering incentive compatibility in the learning from expert advice setting, we are restricted to considering proper scoring rules. However, it is not clear at this point that there are proper scoring rules that could lead to algorithms with small regret. 


